Proposal from the NA61/SHINE Collaboration for update of European Strategy for Particle Physics

Building on the current program's success and driven by new physics challenges, the NA61/SHINE Collaboration proposes to continue measuring hadron production properties in reactions induced by hadron and ion beams after CERN Long Shutdown 3. These measurements are of significant interest to the heavy-ion, cosmic-ray, and neutrino physics communities and will focus on: - Investigating hadron production in the light-ion systems to explore the diagram of high-energy nuclear collisions, and to obtain new insight into the unexpected violation of isospin (flavor) symmetry recently observed by the experiment; - Measuring charm-anticharm correlations to gain unique insights into the production locality of charm and anticharm quark pairs; - Examining strangeness and multi-strangeness production to improve our understanding of the early Universe's evolution and neutron star formation; - Measuring cross sections relevant for cosmic-ray measurements, significantly boosting searches for new physics in our Galaxy; - Conducting hadron production measurements with proton, pion, and kaon beams for neutrino physics, enhancing the precision of hadron production data needed for initial neutrino flux predictions in neutrino oscillation experiments; - Measuring hadron production processes relevant for understanding the flux of atmospheric neutrinos, as well as neutrinos and muons from spallation sources. To achieve these objectives, a detector upgrade and a beam upgrade are required, with data-taking planned for the period 2029-2032 and beyond.

==> include/Makefile <==
# Makefile for generating presentation tex related files
# $Id: Makefile 3154 2013-09-26 15:17:51Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TARGET := na61Preprint
DEPENDENCIES := $(wildcard plots/* *.tex *.bib include/*bib)

##########################################################

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e)print red""e""end;exit !!e}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && exit 0 ; done ; exit 1
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $<
  bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(TARGET).pdf

# dependencies
$(TARGET).pdf: $(DEPENDENCIES)

clean:
	- for e in .tex~ .ps .pdf .dvi .log .toc .nav .out .snm .bbl .blg .spl .lof Notes.bib .maf .fff .lot .ttt ; do rm -f $(TARGET)$$e ; done
	- rm -f *.aux include/*.aux

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf %.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.ps
	ps2pdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> include/na61AuthorsLimited.tex <==
% based on XML DB with time Mon Jul  7 16:27:29 2025
% Authors in alphabetical order.

\noindent
{T.\;Anti\'ci\'c~\href{https://orcid.org/0000-0002-6606-0191}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,1}},
{J.J.\;Back\textsuperscript{\,3}},
{A.\;Bravar\textsuperscript{\,8}},
{N.\;Charitonidis\textsuperscript{\,9}},
{M.\;\'Cirkovi\'c~\href{https://orcid.org/0000-0002-4420-9688}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,10}},
{A.\;De~Roeck\textsuperscript{\,9}},
{F.\;Diakonos\textsuperscript{\,2}},
{S.J.\;Dolan\textsuperscript{\,9}},
{R.A.\;Fernandez\textsuperscript{\,9}},
{K.J.\;Floethner\textsuperscript{\,9}},
{P.\;Ghosh~\href{https://orcid.org/0000-0003-1293-3660}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,4}},
{P.\;Granger\textsuperscript{\,9}},
{A.\;Kapoyannis\textsuperscript{\,2}},
{J.F.\;Krizmanic~\href{https://orcid.org/0000-0002-9690-9352}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,4}},
{M.O.\;Kuttan\textsuperscript{\,5}},
{F.\;Lanni\textsuperscript{\,9}},
{O.\;Linnyk\textsuperscript{\,5}},
{L.\;Munteanu\textsuperscript{\,9}},
{C.\;Mussolini\textsuperscript{\,9}},
{J.\;Pawlowski\textsuperscript{\,5}},
{W.\;Rauch\textsuperscript{\,6}},
{L.\;Scharenberg\textsuperscript{\,9}},
{S.\;Schramm\textsuperscript{\,5}},
{J.\;Steinheimer-Froschauer\textsuperscript{\,5}},
{H.\;Stoecker\textsuperscript{\,5}},
{H.\;Str\"obele\textsuperscript{\,7}},
{T.\;\v{S}u\v{s}a~\href{https://orcid.org/0000-0001-7430-2552}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,1}},
{A.\;Toia~\href{https://orcid.org/0000-0001-9567-3360}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,7}},
{M.\;Vassiliou\textsuperscript{\,2}}, and
{K.\;Zhou\textsuperscript{\,5}}


==> include/na61InstitutionsLimited.tex <==
% based on XML DB with time Mon Jul  7 16:27:29 2025
% Institutes in alphabetical order.

\noindent
\textsuperscript{1}~Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia\\
\textsuperscript{2}~University of Athens, Athens, Greece\\
\textsuperscript{3}~University of Warwick, Warwick, Great Britain\\
\textsuperscript{4}~Goddard Space Flight Center, Greenbelt, USA\\
\textsuperscript{5}~Frankfurt Institute for Advanced Studies, Frankfurt, Germany\\
\textsuperscript{6}~Fachhochschule Frankfurt, Frankfurt, Germany\\
\textsuperscript{7}~University of Frankfurt, Frankfurt, Germany\\
\textsuperscript{8}~University of Geneva, Geneva, Switzerland\\
\textsuperscript{9}~CERN, Geneva, Switzerland\\
\textsuperscript{10}~University of Belgrade, Belgrade, Serbia\\


==> source/objectives/long_term_future_for_measurements_at_SPS.tex <==
{\itshape \color{blue} Coordinator: Marek, Eric}

